DAFT: Distilling Adversarially Fine-tuned Models for Better OOD Generalization

We consider the problem of OOD generalization, where the goal is to train a model that performs well on test distributions that are different from the training distribution. Deep learning models are known to be fragile to such shifts and can suffer large accuracy drops even for slightly different test distributions. We propose a new method - DAFT - based on the intuition that adversarially robust combination of a large number of rich features should provide OOD robustness. Our method carefully distills the knowledge from a powerful teacher that learns several discriminative features using standard training while combining them using adversarial training. The standard adversarial training procedure is modified to produce teachers which can guide the student better. We evaluate DAFT on standard benchmarks in the DomainBed framework, and demonstrate that DAFT achieves significant improvements over the current state-of-the-art OOD generalization methods. DAFT consistently out-performs well-tuned ERM and distillation baselines by up to 6%, with more pronounced gains for smaller networks.

==> sections/analysis.tex <==
We also visually analyzed various classes from the Office Real World dataset where results by \alg differ significantly from baselines. In Table~\ref{tab:classwiseanalysis}, we present examples from four classes, two on which \alg is more accurate than ERM, and two on which it is at par or worse than ERM. We observe that for classes like backpack, the images from the target domain (Real images) are highly similar to some training domain (Product images). This perhaps explains relatively poor performance of \alg compared to ERM.  However, when the images from test/train domains are visually dissimilar, \alg\ can be significantly more accurate than ERM. For example, for the sink class, Real-World images are realistic pictures of sinks while product, Art, ClipArt domains mostly consist of stylized {\em clean} images of sinks. Here \alg is about 20\% more accurate. 
Overall, \alg\ improves on 58 of the 65 classes. %
\begin{table}[!t]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{cc|c|ccc}
    \toprule
    Class     &  Improvement & Target & \multicolumn{3}{|c}{Source}\\
    \hline
    \multirow{2}{*}{Backpack}     & \multirow{2}{*}{-14.1\%} & \includegraphics[width=0.18\columnwidth]{figures/backpack_rw.jpg}  & \multirow{2}{*}{\includegraphics[width=0.2\columnwidth]{figures/backpack_prod.jpg}}&\multirow{2}{*}{\includegraphics[width=0.2\columnwidth]{figures/backpack_art.jpg}} &\multirow{2}{*}{\includegraphics[width=0.2\columnwidth]{figures/backpack_ca.jpg}}\\
     & & \includegraphics[width=0.18\columnwidth]{figures/backpack_rw2.jpg} & & &  \\
    \hline
    \multirow{2}{*}{Flowers}     & \multirow{2}{*}{0\%} & \includegraphics[width=0.18\columnwidth]{figures/flower_rw.jpg}  & \multirow{2}{*}{\includegraphics[width=0.2\columnwidth]{figures/flower_prod.jpg}}&\multirow{2}{*}{\includegraphics[width=0.2\columnwidth]{figures/flower_art.jpg}} &\multirow{2}{*}{\includegraphics[width=0.2\columnwidth]{figures/flower_ca.jpg}}\\
     & & \includegraphics[width=0.18\columnwidth]{figures/flower_rw2.jpg} & & &  \\
    \hline
    \multirow{2}{*}{Trashcan}     & \multirow{2}{*}{7.4\%} & \includegraphics[width=0.18\columnwidth]{figures/trashcan_rw2.jpg}  & \multirow{2}{*}{\includegraphics[width=0.2\columnwidth]{figures/trashcan_prod.jpg}}&\multirow{2}{*}{\includegraphics[width=0.2\columnwidth]{figures/trashcan_art.jpg}} &\multirow{2}{*}{\includegraphics[width=0.2\columnwidth]{figures/trashcan_ca.jpg}}\\
     & & \includegraphics[width=0.18\columnwidth]{figures/trashcan_rw.jpg} & & &  \\
    \hline
    \multirow{2}{*}{Sink}     & \multirow{2}{*}{20.0\%} & \includegraphics[width=0.18\columnwidth]{figures/sink_rw.jpg}  & \multirow{2}{*}{\includegraphics[width=0.2\columnwidth]{figures/sink_prod.jpg}}&\multirow{2}{*}{\includegraphics[width=0.2\columnwidth]{figures/sink_art.jpg}} &\multirow{2}{*}{\includegraphics[width=0.2\columnwidth]{figures/sink_ca.jpg}}\\
     & & \includegraphics[width=0.18\columnwidth]{figures/sink_rw2.jpg} & & &  \\
    
    \bottomrule
    \end{tabular}
    }\vspace*{-10pt}
    \caption{\alg vs  ERM. We show sample images from source and target domains for $4$ of the $65$ classes from Office-Home dataset. \alg performs worse than ERM on Backpack,  have similar performance on Flowers and  outperforms  ERM on Trashcan and Sink class. Visually, part of the source and target domain images are similar for Backpack and Flowers while there is a large variation in the remaining two classes, indicating that \alg tends to outperform ERM when there is a large distribution shift.}\vspace*{-15pt}
    \label{tab:classwiseanalysis}
\end{table}

    

